AU-Aware Vision Transformers for Biased Facial Expression Recognition

Studies have proven that domain bias and label bias exist in different Facial Expression Recognition (FER) datasets, making it hard to improve the performance of a specific dataset by adding other datasets. For the FER bias issue, recent researches mainly focus on the cross-domain issue with advanced domain adaption algorithms. This paper addresses another problem: how to boost FER performance by leveraging cross-domain datasets. Unlike the coarse and biased expression label, the facial Action Unit (AU) is fine-grained and objective suggested by psychological studies. Motivated by this, we resort to the AU information of different FER datasets for performance boosting and make contributions as follows. First, we experimentally show that the naive joint training of multiple FER datasets is harmful to the FER performance of individual datasets. We further introduce expression-specific mean images and AU cosine distances to measure FER dataset bias. This novel measurement shows consistent conclusions with experimental degradation of joint training. Second, we propose a simple yet conceptually-new framework, AU-aware Vision Transformer (AU-ViT). It improves the performance of individual datasets by jointly training auxiliary datasets with AU or pseudo-AU labels. We also find that the AU-ViT is robust to real-world occlusions. Moreover, for the first time, we prove that a carefully-initialized ViT achieves comparable performance to advanced deep convolutional networks. Our AU-ViT achieves state-of-the-art performance on three popular datasets, namely 91.10% on RAF-DB, 65.59% on AffectNet, and 90.15% on FERPlus. The code and models will be released soon.

==> expe.tex <==
In this section, we first describe the implementation details and datasets, and then demonstrate the superiority of AU-ViT in joint training. Finally, we conduct ablation studies and make visualization analysis to show the effectiveness of each component.

\subsection{Implementation details}

For the base branch, the vanilla ViT is pre-trained on VGGFace2~\cite{cao2018vggface2} with image size of 224$\times$224, and the CNN Embedding module is initialized by IR50~\cite{wang2021face} pre-trained on MS1M~\cite{guo2016ms}. We generate pseudo AU labels for the FER datasets by the AU detector OpenFace~\cite{baltrusaitis2018openface}. All the images are aligned and resized to 112$\times$112. For data augmentation, we use Random-Horizontal Flip, Random-Grayscale and Gaussian Blur for all datasets. We use Adam optimizer for RAFDB and FERPlus, and SGD optimizer for AffectNet. The weight decay is 5e-4, and the batch size is 64 for RAFDB, 128 for FERPlus and AffectNet. The learning rate is initialized as 0.0001, and we use a linear learning rate warm-up of 10 epochs and cosine learning rate decay of 10 epochs. All the experiments are implemented by Pytorch with 4 NVIDIA V100 GPUs. The default $\alpha$ and $\beta$ in Equation (\ref{eq:loss}) are 1.0 and 1.0, respectively. 


\renewcommand\arraystretch{2}
\begin{table*}[ht]
\center
\begin{tabular}{c||c|c|c|c|c}
\hline
\diagbox{Target}{Accuracy (\%)}{Auxiliary}         & RAFDB & FERPlus & AffectNet & RAFAU & EmotioNet \\ \hline\hline
RAFDB  & /  & 88.41 (+3.57)    & 87.84 (+1.17)  & \textbf{88.8} (+6.08)   & 87.9 (+2.8)     \\ \hline
FERPlus  & 88.4 (+1.86)  & /  & 88.34 (+0.56)     & 88.44 (+1.25)  &\textbf{88.53} (+1.6)      \\ \hline
AffectNet & 61.57 (+3.38)  & 62.03 (+2.12)  & /  & \textbf{62.33} (+3.09)  & 61.17 (+2.83)  \\
\hline
\end{tabular}
\caption{The results of joint training on dataset pairs with our basic AU-ViT. The numbers in brackets present the improvements of our basic AU-ViT compared to the results of ViT in Table \ref{tab:FER-FER}.}
\label{tab:FER-AU}
\end{table*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{wrong picture.pdf}
\caption{The illustration of predicted samples by vanilla ViT trained on individual datasets and our basic AU-ViT jointly-trained with RAFAU. The red texts indicate incorrect predictions by vanilla ViT while the green ones indicate correct predictions by the AU-ViT.}
\label{fig: Wrong classed}
\end{figure*}

\begin{figure*}[t]
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{CM/ViT on RAF-DB.pdf}  
%   \caption{\small{ViT on RAF-DB.}
%   \label{fig:ViT on RAF-DB}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{CM/ViT on FERPlus.pdf}  
%   \caption{\small{ViT on FERPlus.}}
%   \label{fig:ViT on FERPlus}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{CM/ViT on AffectNet.pdf}  
%   \caption{\small{ViT on AffectNet.}}
%   \label{fig:ViT on AffectNet}
\end{subfigure}
\\
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{CM/AU-ViT on RAF-DB.pdf}
%   \caption{\small{AU-ViT on RAF-DB.}}
%   \label{fig:AU-ViT on RAF-DB}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{CM/AU-ViT on FERPlus.pdf}
%   \caption{\small{AU-ViT on FERPlus.}}
%   \label{fig:AU-ViT on Occlusion-AffectNet}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{CM/AU-ViT on AffectNet.pdf}
%   \caption{\small{AU-ViT on AffectNet.}}
%   \label{fig:AU-ViT on AffectNet}
\end{subfigure}
\caption{The confusion matrices of the vanilla ViT and our AU-ViT on RAF-DB, FERPlus and AffectNet.}
\label{fig: cm of AU-ViT}
\end{figure*}

\subsection{Datasets}
To evaluate our method, we use three popular in-the-wild facial expression datasets, namely RAF-BD~\cite{li2017reliable}, FERPlus~\cite{BarsoumICMI2016} and AffectNet~\cite{mollahosseini2017affectnet}, and two popular in-the-wild facial AU datasets, namely RAFAU~\cite{Yan_2020_ACCV} and EmotioNet~\cite{fabian2016emotionet}. Besides, we also use the occlusion test datasets~\cite{wang2020region} from RAFDB, FERPlus and AffectNet.

\textbf{RAFDB}~\cite{li2017reliable}. It consists of 30,000 facial images that are downloaded from the Internet and are annotated with basic or compound expressions by 40 trained human students. It is a large-scale and real-world dataset. In our experiment, we only use images with seven basic expressions (neutral, happiness, surprise, sadness, anger, disgust, fear, neutral), which includes 12,271 images for training and 3,068 images for test. We mainly report the overall accuracy on the test set.

\textbf{FERPlus}~\cite{BarsoumICMI2016}. The FERPlus contains 28,709 training images, 3,589 validation images and 3,589 test images, which are collected by the Google search engine. All of the images in FERPlus are aligned and resized to 48$\times$48, each of which is annotated by 10 annotators. We re-align the faces in the aligned set of FERPlus to increase the area ratio of faces in an image. Apart from seven basic emotions in FER2013, contempt is included in FERPlus. We mainly report the overall accuracy of the test set. 

\textbf{AffectNet}~\cite{mollahosseini2017affectnet}. The AffectNet is by far the largest dataset that provides both categorical  and Valence-Arousal annotations. It includes more than one million images from the Internet by querying expression-related keywords in three search engines. In AffectNet, about 420,000 images are manually annotated with eight basic expression labels like RAFDB and 3500 validation images. It should be noted that AffectNet has an imbalanced training set and test set as well as a balanced validation set. So we use a oversampling strategy in training phase to produce a balanced batch samples. The overall accuracy on the validation set is used for measurement, where each category contains 500 samples.

\textbf{RAFAU}~\cite{Yan_2020_ACCV}. The RAFAU is an extended dataset of RAF-ML collected from the Internet with blended emotions. It varies in subjects' identity, head poses, lighting conditions and occlusions.
The face images in RAFAU are FACS-coded by two experienced coders independently. It contains 4601 real-world images with 26 kinds of AUs: AU1, AU2, AU4, AU5, AU6, AU7, AU9, AU10, AU12, AU14, AU15, AU16, AU17, AU18, AU20, AU22, AU23, AU24, AU25, AU26, AU27, AU28, AU29, AU35, AU43. In our experients, we only use the first 21 AUs, which have a strong relationship with expressions. 


\textbf{EmotioNet}~\cite{fabian2016emotionet}. The EmotioNet database includes 950,000 images with annotated AUs. The images are downloaded the Internet with related emotion keywords. These images are then automatically annotated with AUs, AU intensities and emotion categories by a specific algorithm. It contains 23 kinds of AUs, including AU1, AU2, AU4, AU5, AU6, AU9, AU10, AU12, AU15, AU17, AU18, AU20, AU24, AU25, AU26, AU28, AU43, AU51, AU52, AU53, AU54, AU55, AU56. In our experiments, we only use the first 16 AUs, which have a strong relationship with expressions.

 \textbf{Occlusion FER datasets}~\cite{wang2020region}. The total numbers of occlusion samples in FERPlus (test set), AffectNet (validation set), and RAF-DB (test set) are respectively 605, 682 and 735, which are 16.86\%, 17.05\%, and 23.9\% of their original sets. These real-world test sets are annotated manually with different occlusion types, which include wearing a mask, wearing glasses, objects on the left/right, objects in the upper face and objects in the bottom face, non-occlusion. Images in the occlusion test sets are with at least one type of occlusions. We mainly report the overall accuracy on the three occlusion datasets.
 
\subsection{Joint training with AU-ViT}


% \begin{table*}[ht]
% \center
% \caption{Ablation study on joint training schemes, performed on RAFDB, FERPlus and AffectNet with different auxiliary AU Datasets. FERPlus* only contains 7 classes without contempt. The AU label of RAFDB, FERPlus and AffectNet are generated by OpenFace\cite{baltrusaitis2018openface}.}
% \label{tab:FER-AU}
% \setlength{\tabcolsep}{4mm}
% \begin{tabular}{ccccccc}
% \toprule
%           & RAFDB & FERPlus* & AffectNet & RAFAU & EmotioNet & Baseline \\ \midrule
% RAFDB    & 87.81 (+0.51)   & 88.41 (+3.57)    & 87.84 (+1.17)  & \textbf{88.8} (+6.08)   & 87.9 (+2.8)   & 87.3     \\ \midrule
% FERPlus*   & 88.4 (+1.86)  & 88.24 (+0.33)  & 88.34 (+0.56)     & 88.44 (+1.25)  &\textbf{88.53} (+1.6) & 87.91    \\ \midrule
% AffectNet & 61.57(+3.38)  & 62.03(+2.12)  & 61.11(+1.06)  & \textbf{62.33}(+3.09)  & 61.17(+2.83)   & 60.05   \\ \bottomrule
% \end{tabular}
% \end{table*}

We conduct extensive joint training experiments among three FER datasets: RAFDB, FERPlus, and AffectNet, and two AU datasets: RAFAU and EmotioNet. In particular, we predict pseudo AUs for FER datasets via OpenFace\cite{baltrusaitis2018openface}. The predicted AUs include AU1, AU2, AU4, AU5, AU6, AU7, AU9, AU10, AU12, AU14, AU15, AU17, AU20, AU23, AU25, and AU26, which are all used for training. Besides, we select available expression-related AUs if auxiliary AU datasets are used. The specific AUs are mentioned in datasets section. In the experiments, similar to Table \ref{tab:FER-FER}, the base branch adopts the vanilla ViT and is pretrained on the VGGFace2~\cite{cao2018vggface2}. The results are shown in Table \ref{tab:FER-AU}.

Compared to joint training with FER labels (i.e., Table \ref{tab:FER-FER}), our AU-ViT significantly enhances the performance, e.g., we achieve 6.08\% gain for RAFDB when combining RAFDB and RAFAU. These results demonstrate the effectiveness of our AU-ViT. We also find other two observations as follows. First, when combining AU datasets, the gain from RAFAU is generally larger than that from EmotioNet, which is consistent with the AU distance in Figure \ref{fig: cosine distance}. Second, the auxiliary AU datasets usually bring more improvements, which may be explained that the manual AU annotations has better quality than the pseudo one. 

%First, as the confusion metrics of baseline shown, easily-confused expression categories are fear and neutral, sadness and disgust, and sadness and anger. Our AU-ViT improves the performance in all easily-confused expression categories compared to the baseline method. For example, in the comparison Occlusion-RAFDB, 14\% of fear samples are recognized as neutral by baseline, while it decreases to 0\% with our method. In confusion-FERPlus and confusion-AffectNet, a considerable part of disgust samples are mistaken for sadness, But in the results of our method, the recall of disgust increases notably. Second, we find that our method consistently boosts the ``happiness'', ``sadness'' and ``anger'' categories on all the test sets. We believe it may be because these facial expressions have noticeable  region features, such as action units of ``Brow lowerer'', ``Cheek Raiser'', and ``Upper lid raiser'', which can be explicitly captured by our AU-ViT. The above results indicate that our AU-ViT is robust in the occlusion-challenge condition.

To investigate the superiority of our AU-ViT, we show the samples which are correctly recognized by AU-ViT but not by ViT in Figure \ref{fig: Wrong classed}. From these samples, we find the AU-ViT perform better in four aspects of samples: inter-class similarity, weak expression, occlusion, and profile. Different expressions sometimes share partial similar facial motions, e.g., a sad face may raise the mouth corner and show the teeth as in a happy face. The ViT trained with FER labels is confused by these samples while the AU-ViT is not. It may be explained by that the AU branch of AU-ViT makes the model pay attentions on all the local regions which are related to action units. Some expressions (e.g., sadness, surprise, and anger) have weak intensity and look similar to neutral. Occlusion and profile faces make it hard for ViT since the critical clues like in front faces are missing. However, our AU-ViT occasionally captures dominated features for expressioin recognition in non-occlusion facial regions thanks to the AU recognition branch.
We further make another comparison between ViT and our basic AU-ViT by illustrating confusion matrices in Figure \ref{fig: cm of AU-ViT}. Our AU-ViT achieves remarkable improvements for the categories `Fear' and `Anger' on RAF-DB, `Disgust' and `Anger' on FERPlus, `Disgust' and `Sadness' on AffectNet.

%The AU-ViT distinguishes neutral and other expressions better than the ViT since the AU branch encourages to capture small motions. (3) Occlusion (e.g., hands, glasses and objects) shelters facial region and makes FER difficult. The pure ViT is disturbed while the AU-ViT keeps accurate. It is because the AU branch takes advantage of all facial regions for auxiliary AU recognition. (4) Profile images show half faces and introduce background. The AV-ViT still identifies expression well since the AU branch seizes the emotional clues from the half face by AU recognition. The above challenging images mainly bring confusion to FER task. The AU-ViT eliminates the challenges through focusing on all the facial regions and capturing the facial motions. This is why the AU-ViT gains improvement while the pure ViT suffers degrade if joint-training carries more difficult samples.




\begin{table}[t]
\center
\caption{Evaluation of advanced modules in AU-ViT. The results are reported on RAFDB, and the AU-ViT models are jointly trained on RAFDB and RAFAU.}
\label{tab:Ablation_All}
% \setlength{\tabcolsep}{4mm}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}cccccc@{}}
\toprule
CNN Embedding   & Multi-stage   & Conv-FFN  & Patch-flatten    & AU Branch & Accuracy  \\
\midrule
                &               &           &                   &           & 87.30     \\
                &               &           &                   &      $\surd$      & 88.80     \\
$\surd$         &               &           &                   &           & 89.86  \\
$\surd$         &$\surd$        &           &                   &           & 90.12 \\
$\surd$         &$\surd$        &$\surd$    &                   &           & 90.22   \\
$\surd$         &$\surd$        &$\surd$    &$\surd$            &           & 90.42  \\
$\surd$         &$\surd$        &$\surd$    &$\surd$            &$\surd$    &\textbf{91.10}  \\
\bottomrule
\end{tabular}}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{visualization.pdf}
\caption{Different attention feature maps from (\uppercase\expandafter{\romannumeral1}) the vanilla ViT, (\uppercase\expandafter{\romannumeral2}) ViT with CNN Embedding, (\uppercase\expandafter{\romannumeral3}) ViT with CNN Embedding and Multi-stage blocks, and (\uppercase\expandafter{\romannumeral4}) our final version of AU-ViT. Each row refers to one of the 7 facial expression on RAFDB.}
\label{fig:visualization}
\end{figure}

\subsection{Advanced modules for AU-ViT}
Though our basic AU-ViT has already obtained comparable performance to state-of-the-art methods, recent advanced modules for Transformers can further be embedded into our AU-ViT. Thus, an evaluation is designed to investigate the effects of CNN Embedding block, Multi-stage block, Conv-FFN, and Patch-flatten operations. The results are presented in Table \ref{tab:Ablation_All}. For the CNN Embedding block in our base branch, we resort to the IR50 pre-trained on the MS1M dataset~\cite{wang2021face} and use the output feature maps from the third stage as input of Transformer blocks. Adding the CNN Embedding block brings the largest gain, i.e., 2.56\%, which can be due to the large-scale pre-trained face dataset or the CNN architecture itself. The Multi-stage Transformer block can capture features from larger regions than normal ViT blocks, which improves the result with CNN Embedding by 0.56\%. To keep more information from the last fully-connected layer, we flatten all patch embeddings instead of simply projecting the class token. This simple change also brings 0.2\% performance gain. It is worth noting that our key AU branch consistently obtains visible gains whether advanced modules are used or not. Our final version of AU-ViT achieves 91.10\% on RAFDB.

% The baseline method (the first line) is the pure ViT with basic size.
% Firstly, we use the former 3 stages of IR50 as our CNN embedding generator and feed patch embeddings into 6 regular Transformer blocks to obtain the classification results. CNN embedding can reach 89.86\% with the weights pre-trained on the MS1M dataset. Multi-stage Transformer can sense larger-scale features than normal ViT, which improves from CNN Embedding by 0.56\%. 
% Conv-FNN contains a 3*3 convolution operation in the FFN layer to enhance the interaction among neighbouring patches with gains 0.1\%.
% To reserve more information to the last fully-connected layer, we flatten all patch embeddings instead of simply projecting the class-token, improved by 0.2\%. 
% AU branch guided the Emotion branch to learn a good representation of AU to improve the performance, which achieves the-state-of-the-art performance of 91.10\%, improved by 0.68\%. So we believe that both the Emotion and AU branches contribute to the good performance of facial expression recognition.
% This may be explained by that this is due by the perception of large-scale features and the interaction with local features, which both help learn good representations of facial expression.



\textbf{Visualization}.
To investigate the effects of each modules, we  employ the ScoreCAM~\cite{2020Score} to visualize the attention feature maps from different models in Figure \ref{fig:visualization}. %To clearly demonstrate, we resize the visualization attention maps to the same size as the original images and highlight attention maps the COLORMAP\_JET color mapping to input faces.
% Fig \ref{fig:visualization} shows the attention maps of seven kinds of facial expressions in RAFDB. The figure has seven rows, each of which shows one of seven categories of expression. 
From (a) to (g), the categories are surprise, fear, disgust, happiness, sadness, anger and neutral. The first column shows the input aligned facial images, and the second to fifth columns show the results of four different models, namely (\uppercase\expandafter{\romannumeral1}) the vanilla ViT, (\uppercase\expandafter{\romannumeral2}) ViT with CNN Embedding, (\uppercase\expandafter{\romannumeral3}) ViT with CNN Embedding and Multi-stage blocks, and (\uppercase\expandafter{\romannumeral4}) our final version of AU-ViT. 

Comparing different columns, we find that adding CNN Embedding can eliminate unrelated attention regions on the face(e.g., (\uppercase\expandafter{\romannumeral1}), (\uppercase\expandafter{\romannumeral2}) in (b) and (d) ). Multi-stage Transformer guides to learn proper and correct features (e.g. (\uppercase\expandafter{\romannumeral2}), (\uppercase\expandafter{\romannumeral3}) in (c)). The AU branch shrinks the attention maps and focuses on more key areas. Take column (\uppercase\expandafter{\romannumeral4}) in (b) for example, the model with AU branch pays attention to the mouth, brow, and eyes while the model without AU branch only focuses on mouth and brow. This visualization can further explain why our AU-ViT outperforms vanilla ViT in the situations of weak expression, occlusion, etc. %For happiness(d), AU branch guides the Emotion branch to focus on the corner of mouth instead of both mouth and eyes like (\uppercase\expandafter{\romannumeral3}), because the changing of eyes is not very important for happiness.

\subsection{Comparison with the state-of-the-art methods}
We compare our final version of AU-ViT to the state-of-the-art methods on RAFDB, FERPlus, and AffectNet.

\begin{table}[tp]
\center
% \setlength{\tabcolsep}{5mm}
\caption{Comparison to the state-of-the-art results on the FERPlus dataset.}
\begin{tabular}{ccccc}
\toprule
Type                        & Method                        & Year      & Public   & Performance \\\midrule
\multirow{5}{*}{CNN}        &PLD\cite{Barsoum2016TrainingDN}&2016       &ICMI       &85.10 \\
                            &SCN\cite{wang2020suppressing}  &2020       &CVPR       &88.01  \\
                            &RAN\cite{wang2020region}       &2020       &CVPR       &88.55  \\
                            &DMUE\cite{she2021dive}         &2021       &CVPR       &89.51 \\ \midrule
\multirow{3}{*}{Transformer}&VTFF\cite{ma2021facial}        &2021       &TAC        &88.81  \\
                            &MVT\cite{li2021mvt}            &2021       &/          &89.22  \\
                            % &TransFER\cite{xue2021transfer}   &2021    &ICCV       &\textbf{90.83}\\
                            &Ours                           &2022       &/          &\textbf{90.15}\\
                            \bottomrule
\end{tabular}
\label{tab:sota_FERPlus}
\end{table}


\textbf{Comparison on FERPlus}.
Table \ref{tab:sota_FERPlus} shows the comparison between our AU-ViT and state-of-the-art methods on FERPlus. Among them, PLD~\cite{Barsoum2016TrainingDN}, SCN~\cite{wang2020suppressing} and RAN~\cite{wang2020region} are CNN-based methods. PLD uses VGG13 as the backbone, which is very simple and light. SCN tends to solve the uncertain problem in the FER task. RAN proposes a region biased loss to encourage high attention weights on the most critical regions.
VTFF~\cite{ma2021facial} and MVT~\cite{li2021mvt} are Transformer-based methods. VTFF also utilizes CNN embeddings and a multi-layer transformer encoder to recognize expressions. MVT uses two Transformer modules to filter out useless patches and classify the remain features, respectively. Our elaborately-designed AU-ViT outperforms these state-of-the-art methods and achieves the accuracy of 90.15\%.
% The AU-ViT outperforms state-of-the-art methods and achieves an accuracy of 90.15\%.
% As shown in Figure \ref{fig: AU-to-emotion bias} in section \ref{method}, the FERPlus has stronger facial motion than the one of other datasets, 
% The images of FERPlus are grey scale, resulting in the loss of detail of facial motion. Because the FERPlus is more similar with RAF-AU than the other two FER datasets, shown in Figure \ref{fig: cosine distance} in the Section \ref{method}, we slightly increase the weight of the loss for AU recognition $\beta$ from 0.5 to 0.8 to increase sensitivity of facial movements.
% Our AU-ViT outperforms state-of-the-art methods and achieves an accuracy of 90.15\%.

\begin{table}[tp]
\center
% \setlength{\tabcolsep}{5mm}
\caption{Comparison to the state-of-the-art results on the AffectNet-7 dataset.}
\begin{tabular}{ccccc}
\toprule
Type                        & Method                        & Year      & Public   & Performance \\
\midrule
\multirow{5}{*}{CNN}        &IPA2LT~\cite{zeng2018facial}    &2018       &ECCV       &57.31 \\
                            &LDL-ALSG~\cite{chen2020label}   &2020       &CVPR       &59.35 \\
                            &DDA-Loss~\cite{Farzaneh_2020_CVPR_Workshops} &2020&CVPR &62.34 \\
                            &DMUE~\cite{she2021dive}        &2021    &CVPR           &63.11 \\
                            &EfficientFace~\cite{zhao2021robust} &2021   &AAAI       &63.7 \\
                            &KTN~\cite{2021Adaptively}       &2021       &TIP        &63.97 \\
                            &Meta-Face2Exp~\cite{zeng2022face2exp}  &2022&CVPR       &64.23 \\
                            &DACL~\cite{farzaneh2021facial}  &2021       &WACV       &65.20 \\ 
                            \midrule
\multirow{3}{*}{Transformer}&MVT~\cite{li2021mvt}            &2021       &/          &64.57 \\
                            &VTFF~\cite{ma2021facial}        &2021       &TAC        &64.80 \\
                            % &TransFER~\cite{xue2021transfer}   &2021    &ICCV       & \textbf{66.23}\\
                            &Ours                           &2022       &/          &\textbf{65.59} \\
                            \bottomrule
\end{tabular}
\label{tab:sota_AffectNet}
\end{table}

\textbf{Comparison on AffectNet}.
Table \ref{tab:sota_AffectNet} compares our method to several state-of-the-arts methods on AffectNet.
DDA-Loss~\cite{Farzaneh_2020_CVPR_Workshops} optimizes the embedding space for extreme class imbalance scenarios. 
EfficientFace~\cite{zhao2021robust} focuses on label distribution learning.
KTN~\cite{2021Adaptively} designs a distillation strategy to classify highly similar representations.
DACL~\cite{farzaneh2021facial} focuses on the most discriminative facial regions and features.
% To tackle the imbalance problem, we also apply the oversampling strategy in our experiments and obtain 65.59\%.
Due to the gap between the imbalanced training set and the balanced validation set, we also use the traditional oversampling strategy and increase the proportion of auxiliary data in each iteration from 4:1 to 3:1. We finally obtain 65.59\% on AffectNet which outperforms the Transformer-based VTFF by 0.79\%. %to capture more universal AU representation. 
\begin{table}[t] 
\center
% \setlength{\tabcolsep}{5mm}
\caption{Performance comparison with the state-of-the-art methods on RAF-DB.}
\begin{tabular}{ccccc}
\toprule
Type                        & Method                        & Year      & Public   & Performance \\
\midrule
\multirow{5}{*}{CNN}        &DLP-CNN~\cite{2017Reliable}     &2016       &CVPR       & 84.13  \\
                            &LDL-ALSG~\cite{chen2020label}   &2020       &CVPR       & 85.53 \\
                            &IPA2LT~\cite{zeng2018facial}    &2018       &ECCV       & 86.77 \\
                            &RAN~\cite{wang2020region}       &2020       &CVPR       & 86.90 \\
                            &SPDNet~\cite{2018Covariance}     &2018        &CVPRW    & 87.00\\
                            &DDL~\cite{2020Deep}         &2020           &CVPR       & 87.71  \\
                            &SCN~\cite{wang2020suppressing} &2020        &CVPR       & 88.14  \\
                            &Meta-Face2Exp~\cite{zeng2022face2exp}  &2022&CVPR       & 88.54 \\
                            &DMUE~\cite{she2021dive}        &2021    &CVPR           & 89.42 \\
                            &FDRL~\cite{ruan2021feature}    &2021    &CVPR           & 89.72 \\
                            \midrule
\multirow{3}{*}{Transformer}&VTFF~\cite{ma2021facial}        &2021       &TAC        & 88.81 \\
                            &MVT~\cite{li2021mvt}            &2021       &/          & 89.22 \\
                            &TransFER~\cite{xue2021transfer}   &2021    &ICCV       & 90.91\\
                            &Ours                           &2022       &/          &\textbf{91.10}\\
                            \bottomrule
\end{tabular}
\label{tab:sota_RAFDB}
\end{table}


\begin{table}[tp]
\center
\setlength{\tabcolsep}{5mm}
\caption{Comparison between our AU-ViT and other methods with occlusion conditions.}
\begin{tabular}{ccc}

\toprule
Test datasets           & Model     & Acc.    \\\midrule
\multirow{4}{*}{Occlusion-RAFDB}     & ViT(Baseline)  & 81.63 \\
                            & RAN~\cite{wang2020region}        & 82.72  \\
                            & ASF-CVT~\cite{ma2021robust}   & 83.95  \\
                            & AU-ViT    & \textbf{88.02} \\\midrule
\multirow{4}{*}{Occlusion-FERPlus}    & ViT(Baseline)  & 81.48 \\ 
                            & RAN~\cite{wang2020region}        & 83.63  \\
                            & ASF-CVT~\cite{ma2021robust}   & \textbf{84.79}  \\
                            & AU-ViT    & \textbf{84.79} \\\midrule
\multirow{4}{*}{Occlusion-AffectNet}  & ViT(Baseline)  & 57.26 \\ 
                            & RAN~\cite{wang2020region}       & 58.50  \\
                            & ASF-CVT~\cite{ma2021robust}   & 62.98  \\
                            & AU-ViT    & \textbf{63.92} \\\bottomrule
\end{tabular}
\label{tab:occlusion}
\end{table}

\textbf{Comparison on RAFDB}.
Table \ref{tab:sota_RAFDB} compares our approach with previous state-of-the-art methods on RAFDB. 
Among all the competing methods, DDL~\cite{2020Deep} and RAN pay attention to disentangling the disturbing factors in facial expression images. SPDNet~\cite{2018Covariance} introduces a new network architecture, and DLP-CNN~\cite{2017Reliable} uses a novel loss function to explore intra-class variations. IPA2LT~\cite{zeng2018facial} and SCN~\cite{wang2020suppressing} try to reduce the effects of noise labels. TransFER~\cite{xue2021transfer} is the first Transformer-based model for the FER task. It is worth noting that IPA2LT also resort to multiple facial datasets for performance boosting via multiple predicted pseudo FER labels from varied models. 
All the above methods improve FER performance by focusing on facial expression images, model architectures, and FER labels, neglecting the importance of AUs. Our AU-ViT finally achieves 91.10\% on RAFDB which surpasses TransFER slightly, establishing a new state of the art .
% TransFER achieves the second-best performance on RAFDB with 90.91\%. Our proposed approach surpasses it to reach 91.10\%, which is a new state of the art to our knowledge.

\textbf{Comparison on occlusion datasets}
As shown in Figure \ref{fig: Wrong classed}, our AU-ViT works better than ViT in occlusion and profile faces thanks to the guidance of AU branch. To further verify this, we evaluate our basic AU-ViT (without advanced modules) on the occlusion test sets of RAFDB, FERPlus and AffectNet. All the models are pretrained on VGGFace2~\cite{cao2018vggface2} and fine-tuned on the corresponding training set. The evaluation results are shown in Table~\ref{tab:occlusion}.% Particularly, the B-branch adopts pure ViT pretrained on VGGFace2~\cite{cao2018vggface2} and is fine-tuned on FER images. 

Two observations can be concluded as follows. First, our AU-ViT improves the baseline ViT significantly on all datasets, with gains of 6.39\%, 3.31\% and 6.66\% on Occlusion-RAFDB, Occlusion-FERPlus and Occlusion-AffectNet, respectively. Second, though ASF-CVT utilizes Transformers on CNN feature maps, our basic AU-ViT still outperforms it on Occlusion-RAFDB and Occlusion-AffectNet with large margins. 
Worth mentioning that the symmetric maxout layer in AU branch can effectively capture AU activation even if half of the face is occluded. We experimentally find that the symmetric maxout layer can consistently bring around 0.5\% performance gain in these experiments.
%The AU-ViT can capture expression more effectively since it pays more attention to the activation of local AUs. Worth mentioning that the symmetric maxout layer of the AU Branch can capture AU activation when half of it is occluded. 


\begin{table*}[t]
\center
% \setlength{\tabcolsep}{5mm}
\caption{Performance comparison between the AU Token and the AU branch on RAFDB.}
\begin{tabular}{c|ccccccc}
\hline
\diagbox{Target}{Accuracy (\%)}{Auxiliary}                     &  &RAFDB  &FERPlus& AffectNet   &RAFAU & EmotioNet &Baseline \\\hline
\midrule
\multirow{2}{*}{RAFDB} &AU token  &87.35  &87.71      & 87.65     &87.97  &87.03 &\multirow{2}{*}{87.3}\\
                                           &AU branch &87.81  &88.41      & 87.84     &88.8   &87.9  &\\
\bottomrule
\end{tabular}
\label{tab:Token_vs_Branch}
\end{table*}


% \begin{figure*}[ht]
% \captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{CM on RAFDB(occlusion)_baseline.pdf}  
%   \caption{\small{Baseline on Occlusion-RAFDB.}}
%   \label{fig:Baseline on Occlusion-RAFDB}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{CM on FERPlus(occlusion)_baseline.pdf}  
%   \caption{\small{ Baseline on Occlusion-FERPlus.}}
%   \label{fig:Baseline on Occlusion-FERPlus}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{CM on AffectNet(occlusion)_baseline.pdf}  
%   \caption{\small{Baseline on Occlusion-AffectNet.}}
%   \label{fig:Baseline on Occlusion-AffectNet}
% \end{subfigure}

% \caption{The confusion  matrices of baseline methods and our AU-ViT on the Occlusion- and Pose-FERPlus test sets.}
% \label{fig:confusion_metrics_baseline}
% \end{figure*}


% \begin{figure*}[ht]
% \captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{Confusion matrix on RAFDB(occlusion).pdf}  
%   \caption{\small{AU-ViT on Occlusion-RAFDB.}
%   \label{fig:AU-ViT on Occlusion-RAFDB}}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{Confusion matrix on FERPlus(occlusion).pdf}  
%   \caption{\small{AU-ViT on Occlusion-FERPlus.}}
%   \label{fig:AU-ViT on Occlusion-FERPlus}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{Confusion matrix on AffectNet(occlusion).pdf}  
%   \caption{\small{AU-ViT on Occlusion-AffectNet.}}
%   \label{fig:AU-ViT on Occlusion-AffectNet}
% \end{subfigure}
% \caption{The confusion matrices of our AU-ViT on the Occlusion test sets of RAFDB,FERPlus and AffectNet.}
% \label{fig:confusion_metrics_our}
% \end{figure*}



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Ablation pictures/AU Branch.pdf} 
    \caption{Evaluation of the AU branch position in our basic AU-ViT.}
    \label{fig:position}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Ablation pictures/AU patches.pdf} 
    \caption{Evaluation of the splitting strategy in AU branch of our final AU-ViT.}
    \label{fig:split}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{AU patches.pdf}
\caption{Evaluation of different patch-splitting strategies.}
\label{fig:patch splitting}
\end{figure*}


% \begin{figure*}[ht]
% \captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{num_transformer_block.png}  
%   \caption{\small{(a)}}

% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{middle_layer.png}  
%   \caption{\small{(b)}}

% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth]{AU patches.png}  
%   \caption{\small{(c)}}

% \end{subfigure}

% \caption{(a) The evaluation of the number of Transformer blocks. (b) Evaluation of different middle layer in ViT from where AU branch extends. (c) Evaluation of different number of patch-splitting. }
% \label{fig:ablation}
% \end{figure*}


% \begin{figure}[t]
% \center
% \includegraphics[width=0.95\linewidth]{num_transformer_block.png}
% \caption{The evaluation of the number(B) Transformer block on RAFDB.}
% \label{fig:Transformer_block}
% \end{figure}
\subsection{Ablation study}
Adding AU information in FER training is previously used for cross-domain facial expression recognition~\cite{wang2020guided} or compound expression recognition~\cite{pu2021expression}. Indeed, it is not trivial to boost performance on individual FER datasets with AUs. Here, we make ablation experiments to show our efforts on this issue.

\textbf{The usage of AUs}.
With AUs, the simple idea is to improve a FER model with multi-task training strategy. Following the idea, we add an AU Token in the baseline ViT and conduct multi-task training on RAFDB with other auxiliary datasets. Specifically, we concatenate the AU token with patch embeddings and the class Token after the linear projection. We implement a multi-layer perception on the AU Token to estimate AUs, and the others are the same as baseline ViT. Table \ref{tab:Token_vs_Branch} presents a comparison between these two usage of AUs. It is worth noting that we can also use the pseudo AUs of RAFDB for training. From Table \ref{tab:Token_vs_Branch}, several observations can be concluded as follows. First, compared to the baseline, the `AU token' multi-task training method can also slightly improve performance except for training with EmotioNet. Second, our AU branch consistently improves the baseline with visible margins. Third, our AU branch not only boosts performance with all auxiliary datasets, but also outperforms the 'AU token' strategy. Thus, we believe that our elaborately-designed AU branch with patch splitting and symmetric maxout can be more precise than just adding an AU token for AU estimation. 

%Moreover, we further compare the performance between AU Token and AU Branch on the RAF-DB. For the vanilla ViT with the AU Token, we concatenate the AU toke with the patch embeddings and the class Token after the linear projection. For the AU recognition, we implement a multi-layer perception on the AU Token of the last Transformer block to obtain the final results. For the vanilla ViT with the AU Branch, we implement the AU Branch on the embeddings of the next-to-last block. As shown in Table~\ref{tab:Token_vs_Branch}, there is a fluctuation in the performance when using the AU Token, especially joint training with the RAF-DB and the EmotioNet. On the contrary, the AU Branch outperforms the baseline consistently. We think the AU Token tends to learn the global representation like the class token for the expression. However, the AU Branch recognizes the AU according to the corresponding area of face which makes the recognition more clear and precise.
%Therefore, we believe the AU Branch can improve more than AU Token in general.

\textbf{The position of AU branch.}
In our AU-ViT model, the base branch and Exp-ViT branch owns 12 Transformer blocks in succession, and our AU branch is extended from the default 10-th block. To investigate the effect of AU branch position, we conduct an evaluation on RAFDB with auxiliary RAFAU by setting the position from 1 to 12, and show the results in Figure \ref{fig:position}. Adding the AU branch in early blocks can be harmful which may be explained by that the early blocks do not have enough semantic information for AU estimation thus can disturb the low-level feature learning for FER. As the AU branch position goes deep, the performance is gradually improved and saturated at the default position. Extending from the last two blocks may slightly damage the semantic features of FER, leading to performance degradation.

% As we introduce in section 3, we extract the patch-tokens from the middle layer in the Emotion branch and then feed them into the AU branch. To explore which layer is best for learning AU features, we evaluate the middle layer M from 1 to 12 on RAFDB. To ensure the resolution of the feature map in each block are equal, we use normal ViT as the whole Emotion branch and set 12 Transformer blocks in it as same as the basic-size ViT, which is considered as the baseline with the accuracy of 87.3\%.

% As (b) of the Figure \ref{fig:ablation} shown, extracting the patch-tokens from the first block drops the performance from the baseline dramatically. As the layer goes deepen, the accuracy is on the rise in general. The peak of accuracy occurs at block 10 while it starts to decrease. We think ViT processes basic features like texture and shape of the face in former blocks. Forcing ViT to learn AU representation too early may destroy the basic feature, which does harm to the performance. On the contrary, guiding ViT to perceive AU too late, like extending in the last block, also impact the performance. Clearly, block 10 is the most suitable one to represent the AU feature.

% \begin{figure}[t]
% \center
% \includegraphics[width=1\linewidth]{middle_layer.png}
% \caption{Evaluation of different middle layer in ViT where AU branch extends from on RAFDB.}
% \label{fig:middle layer}
% \end{figure}

% \begin{figure}
% \center
% \includegraphics[width=1\linewidth]{AU patches.png}
% \caption{Evaluation of different number of patch-splitting on RAFDB.}
% \label{fig:patch-splitting}
% \end{figure}

\textbf{The patch splitting strategy.}
Since AUs are defined as the movement of muscles in face, they naturally are related to local regions. We believe that splitting a face image into different patches is helpful for recognizing AUs. However, it is unknown that which splitting scheme is the best for the final  performance. To this end, we design five schemes for our default AU branch, as shown in Figure \ref{fig:patch splitting}. The splitting schemes namely generate 2, 3, 5, 7, 9 regions for each face image. We do not split the bottom half face in most of the schemes since 14 AUs are related to the lower part of face and it is difficult to separate for individual AUs. All the patches are slightly overlapped for the necessity of complete AU-related features. 

We conduct an evaluation with our final version of AU-ViT and present the results in Figure \ref{fig:split}. Without splitting (i.e., 1 patch), our AU-ViT obtains 90.09\%. It slightly improves performance by splitting into 2 or 3 patches in row. Further splitting the upper face in row and column dramatically boost the accuracy. We get the best performance by the default 7-patch splitting strategy. We observe a visible performance degradation when further splitting the bottom face. All in all, splitting the feature maps into multiple patches keeps spatial information and is helpful for AU estimation and the final FER performance.
% To explore the impact of the number of splitting patches in the AU branch, we evaluate different patch-splitting schemes. Inspired by the above AU branch extending study, we extract the patch-tokens after the third-to-last block.

% The patch-splitting strategies are shown in Figure \ref{fig:patch splitting}. We evaluate the number of patches $P=1,2,3,5,7,9$ on RAFDB. When $P=2,3,5,7,9$, we don't split the bottom patch except the 9-patches partition, because 14 kinds of AU(10, 12, 14, 15, 16, 17, 18, 20, 22, 23, 24, 25, 26, 27) are related to the lower part of face, which is difficult to separate. For 2 patches, we just split into the upper and the lower part. For 3 patches, the upper part of the face can be divided into the top and middle patches. For 5 patches, the middle patch is separated into the left cheek, nose and right cheek. For 7 patches, the top patch is divided into the left eye, brow and right eye. For 9 patches, we divide the bottom patch into the left corner of mouth, the lips and the right corner of mouth. All the patches are overlapped because of the necessity of redundant features.

% The evaluation results are shown in (c) of Figure \ref{fig:ablation}. Firstly, we obtain the baseline 90.09\%, which does not split the feature map. As the number of patches increases, the accuracy rises gradually and goes up dramatically when $P=5$. The 7-patch partition achieves the best performance with an accuracy 91.10\%, outperforming the baseline by 1.01\%. Finally, the performance decreases considerably when $P=9$. Therefore, we believe the multi-patch partition for AU recognition can effectively guide the emotion branch to the critical expression feature.

% \textbf{The number of Transformer blocks.}
% As described in section 3, we utilize several Transformer blocks after the CNN embedding layer. As shown in (a) of Figure~\ref{fig:ablation}, to explore the impact of block number B, we evaluate the B from 1 to 18 on RAFDB with other parameters as default. It must be pointed out that we also drop the AU branch like the above ablation study. The evaluation results are illustrated in Figure 1. As B increases, the performance increases and then decreases after B=6. We think the increase of performance in the beginning is due to the enhancement of representational ability for changing in the face, while the performance decreases gradually because of over-fitting.




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{AU_attn.png}
%     \caption{Evaluation of different attention strategies.}
%     \label{fig:AU_attn}
% \end{figure}
% \subsection{Evaluation of different patch-attention schemes for AU branch}
% To explore the proper architecture for AU branch,we compare different patch-attention schemes,including non-attention, pre-attention,post-attention, pre\&post-attention and cls-attention(number of block from 1 to 4).To avoid the effect of other modules, we use the normal ViT without CNN embedding. Non-attn denotes there are no Attention blocks in the AU branch. Pre-attention denotes an Attention block set before the patch-splitting layer, while post-attention means an Attention block is set after that. Pre\&post-attention scheme both set Attention before and after the patch-splitting layer. Cls-attention denotes each splitting-patch concatenates an AU class token, and then is fed into L Attention blocks(L is equal from 1 to 4).

% The evaluation results are shown in Figure \ref{fig:AU_attn}. We find that Pre, Post and Pre\&Post Attention cannot help improve performance. Class-token Attention schemes cannot reach the performance of Non-attention either. We think employing an additional attention scheme may impair the AU spacial information, which is transferred back from AU labels. Therefore, for AU-ViT, we keep the AU branch as simple as possible, leading the middle layer of the Emotion branch to perceive the AU spacial feature directly.


